GLUE-X: Evaluating Natural Language Understanding Models from an Out-of-distribution Generalization Perspective

Pre-trained language models (PLMs) are known to improve the generalization performance of natural language understanding models by leveraging large amounts of data during the pre-training phase. However, the out-of-distribution (OOD) generalization problem remains a challenge in many NLP tasks, limiting the real-world deployment of these methods. This paper presents the first attempt at creating a unified benchmark named GLUE-X for evaluating OOD robustness in NLP models, highlighting the importance of OOD robustness and providing insights on how to measure the robustness of a model and how to improve it. The benchmark includes 13 publicly available datasets for OOD testing, and evaluations are conducted on 8 classic NLP tasks over 21 popularly used PLMs, including GPT-3 and GPT-3.5. Our findings confirm the need for improved OOD accuracy in NLP tasks, as significant performance degradation was observed in all settings compared to in-distribution (ID) accuracy.

==> tables/tb-rational.tex <==
% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Model}  & \textbf{Precision} & \textbf{Recall} & \textbf{F1}\\ \midrule
% ELECTRA-small   & \textbf{20.95} & \textbf{16.77}     & \textbf{36.61}  \\
% ELECTRA-large   & 20.06 & 15.97     & 36.23  \\
% BERT-large      & 18.67 & 14.54     & 35.11  \\
% T5-large        & 17.96 & 14.20      & 32.80   \\
% ALBERT-base     & 17.37 & 13.60      & 32.00     \\
% T5-base         & 17.19 & 13.85     & 31.02  \\
% T5-small        & 17.15 & 13.79     & 30.32  \\
% ELECTRA-base    & 17.11 & 13.56     & 30.62  \\
% BART-base       & 16.93 & 13.65     & 30.15  \\
% BERT-base       & 16.26 & 12.91     & 30.01  \\
% BART-large      & 16.00    & 12.66     & 29.37  \\
% XLNet-large     & 15.12 & 11.85     & 28.25  \\
% DistilBERT-base & 15.08 & 12.00        & 27.37  \\
% GPT2-medium     & 14.35 & 11.80      & 25.5   \\
% GPT2-large      & 14.35 & 11.64     & 26.35  \\
% RoBERTa-base    & 14.25 & 11.12     & 27.45  \\
% GPT2            & 14.24 & 11.76     & 24.67  \\
% XLNet-base      & 13.63 & 10.91     & 24.94  \\
% RoBERTa-large   & 10.50  & 8.17      & 20.81  \\
% \bottomrule
% \end{tabular}
% \caption{Rationale overlap sorted by the descending order based on the OOD test of sentiment analysis.}
% \label{tab:rationale}
% \end{table}

==> tables/tb-rationale_amazon.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Model}  & \textbf{Precision} & \textbf{Recall} & \textbf{F1}\\ \midrule
ELECTRA-large   & 15.58     & 56.48  & 22.75 \\
ELECTRA-small   & 15.21     & 52.49  & 21.93 \\
T5-large        & 14.1      & 50.68  & 20.55 \\
BERT-large      & 13.38     & 50.04  & 19.76 \\
ALBERT-base     & 13.42     & 48.91  & 19.57 \\
T5-base         & 13.38     & 48.45  & 19.43 \\
ELECTRA-base    & 13.24     & 48.18  & 19.37 \\
BART-large      & 12.7      & 47.38  & 18.71 \\
BART-base       & 12.48     & 45.99  & 18.3  \\
T5-small        & 12.59     & 44.81  & 18.26 \\
BERT-base       & 12.32     & 45.61  & 18.09 \\
RoBERTa-base    & 12.04     & 46.74  & 17.82 \\
XLNet-large     & 11.83     & 45.27  & 17.46 \\
DistilBERT-base & 11.49     & 41.77  & 16.75 \\
XLNet-base      & 10.99     & 41.37  & 16.12 \\
GPT2-medium     & 10.97     & 40.49  & 16.05 \\
GPT2-large      & 10.71     & 40.06  & 15.71 \\
GPT2            & 10.59     & 38.57  & 15.4  \\
RoBERTa-large   & 9.6       & 38.99  & 14.38   \\
\bottomrule
\end{tabular}
\caption{Rationale overlap sorted by the descending order based on the OOD test of sentiment analysis on IMDb dataset.}
\label{tab:rationale_amazon}
\end{table}

==> tables/tb-rationale_imdb.tex <==
\begin{table}[t]
\center
\small
\begin{tabular}{lccc}
\toprule
\textbf{Model}  & \textbf{Precision} & \textbf{Recall} & \textbf{F1}\\ \midrule
ELECTRA-large   & 13.48     & 35.89  & 18.16 \\
ELECTRA-small   & 13.68     & 34.29  & 18.11 \\
T5-base         & 12.16     & 31.59  & 16.09 \\
ALBERT-base     & 11.86     & 31.87  & 15.93 \\
BERT-large      & 11.65     & 32.48  & 15.91 \\
ELECTRA-base    & 11.36     & 29.35  & 15.22 \\
T5-large        & 11.19     & 31.04  & 15.18 \\
BART-base       & 11.26     & 29.33  & 14.99 \\
T5-small        & 11.2      & 28.05  & 14.73 \\
BART-large      & 10.69     & 29.82  & 14.48 \\
BERT-base       & 10.6      & 28.29  & 14.2  \\
XLNet-large     & 9.75      & 27.1   & 13.17 \\
DistilBERT-base & 9.41      & 24.46  & 12.53 \\
GPT2-large      & 9.2       & 24.34  & 12.18 \\
RoBERTa-base    & 8.91      & 25.22  & 12.11 \\
GPT2-medium     & 8.88      & 22.18  & 11.56 \\
XLNet-base      & 8         & 21.88  & 10.72 \\
GPT2            & 8.1       & 19.89  & 10.57 \\
RoBERTa-large   & 6.64      & 20.31  & 9.31   \\
\bottomrule
\end{tabular}
\caption{Rationale overlap sorted by the descending order based on the OOD test of sentiment analysis on IMDb dataset.}
\label{tab:rationale_imdb}
\end{table}

==> tables/tb-rationale_yelp.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Model}  & \textbf{Precision} & \textbf{Recall} & \textbf{F1}\\ \midrule
ELECTRA-small   & 16.62     & 40.67  & 21.58 \\
ELECTRA-large   & 14.76     & 39.52  & 19.78 \\
ALBERT-base     & 14.09     & 37.52  & 18.79 \\
BERT-large      & 13.88     & 38.46  & 18.75 \\
ELECTRA-base    & 14        & 35.66  & 18.38 \\
XLNet-large     & 13.31     & 36.77  & 17.9  \\
T5-large        & 13.04     & 35.56  & 17.49 \\
BERT-base       & 12.98     & 34.6   & 17.31 \\
BART-base       & 12.72     & 34.97  & 17.09 \\
T5-base         & 12.53     & 33.9   & 16.75 \\
T5-small        & 12.3      & 33.37  & 16.47 \\
BART-large      & 11.65     & 31.49  & 15.55 \\
RoBERTa-base    & 11.08     & 30.9   & 14.9  \\
GPT2-large      & 10.8      & 30.21  & 14.42 \\
DistilBERT-base & 10.78     & 29.39  & 14.37 \\
GPT2-medium     & 10.75     & 29.37  & 14.21 \\
XLNet-base      & 10.59     & 29.45  & 14.2  \\
GPT2            & 10.2      & 27.13  & 13.35 \\
RoBERTa-large   & 7.54      & 24.36  & 10.65   \\
\bottomrule
\end{tabular}
\caption{Rationale overlap sorted by the descending order based on the OOD test of sentiment analysis on YELP dataset.}
\label{tab:rationale_yelp}
\end{table}
